Dynamic Hard Pruning of Neural Networks at the Edge of the Internet

Neural Networks (NN), although successfully applied to several Artificial Intelligence tasks, are often unnecessarily over-parametrised. In edge/fog computing, this might make their training prohibitive on resource-constrained devices, contrasting with the current trend of decentralising intelligence from remote data centres to local constrained devices. Therefore, we investigate the problem of training effective NN models on constrained devices having a fixed, potentially small, memory budget. We target techniques that are both resource-efficient and performance effective while enabling significant network compression. Our Dynamic Hard Pruning (DynHP) technique incrementally prunes the network during training, identifying neurons that marginally contribute to the model accuracy. DynHP enables a tunable size reduction of the final neural network and reduces the NN memory occupancy during training. Freed memory is reused by a \emph{dynamic batch sizing} approach to counterbalance the accuracy degradation caused by the hard pruning strategy, improving its convergence and effectiveness. We assess the performance of DynHP through reproducible experiments on three public datasets, comparing them against reference competitors. Results show that DynHP compresses a NN up to $10$ times without significant performance drops (up to $3.5\%$ additional error w.r.t. the competitors), reducing up to $80\%$ the training memory occupancy.

==> trackchanges_AP_input.tex <==
%!TEX root =  ./paper.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%																								%
% Inclusion of packages for todo notes and track changes										%
%																								%
% For todonotes, the only required actions by an author are										%
%   1.  enable -->  before inputting this file                                                  %
%                   a.  define the macro TRACKON, via                                           %
%                       \def\TRACKON{}                                                          %
%                   b.  define the macro TCTEXTWIDTH, via                                       %
%                       \def\TCTEXTWIDTH{XXmm}, where XX is the desired width of the text in mm %
%                       default = \DEFAULTCTEXTWIDTH (if the macro is not defined)              %
%                       NB. This is set ONLY if TRACKON is defined                              %
%                   c. define the width of the margin for notes, via                            %
%                       \def\MARGINNOTES{XXmm}, where XX is the desired width of the notes in mm%
%                       default = \DEFAULTMARGINNOTES (if the macro is not defined              %
%                                                                                               %
%   2. disable -->  make sure TRACKON is not defined                                            %
%																								%
% For track changes, the only required action by an author is 									%
%	1. 	to either enable or disable marking of changes:											%
%		enable --> \usepackage[]{changes}														%
%		disable --> \usepackage[final]{changes}													%
%																								%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\ifdefined\TRACKON
% notes ON
    \usepackage[]{todonotes}
\else
% notes OFF
    \usepackage[disable]{todonotes}
\fi

% Adjust the margins, and the size of the notes in the margin.
\usepackage{setspace}
% set the width of the text, only if track changes is enabled
\ifdefined\TRACKON
    \def\DEFAULTCTEXTWIDTH{150mm}
    \ifdefined\TCTEXTWIDTH
        \setlength{\textwidth}{\TCTEXTWIDTH}
    \else
        \setlength{\textwidth}{\DEFAULTCTEXTWIDTH}
    \fi
\fi

% set the width of the margin notes
\def\DEFAULTMARGINNOTES{20mm}
\ifdefined\MARGINNOTES
    \newcommand{\marginNotesWidth}{\MARGINNOTES}
\else
    \newcommand{\marginNotesWidth}{\DEFAULTMARGINNOTES}
\fi
\setlength{\marginparwidth}{\marginNotesWidth}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\ifdefined\TRACKON
% track changes ON
    \usepackage[]{changes}
\else
% track changes OFF
    \usepackage[final]{changes}
\fi


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% for colors
\usepackage{soul}
\ifdefined\TRACKON
% highlights ON  
    \sethlcolor{yellow}
\else
% highlights in white (for the final text)
    \sethlcolor{white}
\fi


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%																								%
% Definitions for authors.																		%
% This is the only place an author should modify, to pick their own initials and marking color	%
%																								%
% Each author should																			%
% 1. decide which ID to take among the following ones											%
%		replace your favorite 2-letter ID below, e.g.											%
%		change \newcommand{\AIid}{AA} to \newcommand{\AIid}{AP}									%
%		if you want to use AP as your ID														%
%		UP TO YOU GUARANTEE UNIQUENESS OF IDs ACROSS AUTHORS !!!!!!								%
% 2. define the color of your marks																%
%		change \newcommand{\AIcol}{purple} to \newcommand{\AIcol}{blue}							%
%		if you (i) you are author 1 and (ii) you want to use blue								%
%		UP TO YOU GUARANTEE UNIQUENESS OF COLORS ACROSS AUTHORS !!!!!!							%
% 3. stick to use the corresponding commands for add, rep, del, cmt, todo						%
%																								%
% Example commands for author 4 would be														%
% \addAD, \repAD, \cmtAD, \todoInAD etc.														%
%																								%
%																								%
% In more details, this is how you will use the commands										%
% (examples assume the author uses AP as ID)				 									%
% NOTE: unfortunately, those commands do not work with more than one paragraph,					%
% 		so use \\ instead																		%
%																								%
%	trackchanges commands																		%
%	\addAP{new text}																			%
%	\delAP{text to be deleted}																	%
%	\repAP{new text}{text to be deleted}														%
%																								%
%	annotation commands																			%
%	\todoAP{margin comment text} to add a comment in the margin									%
%	\todoInAP{comment text} to add a comment inline												%
%	\cmtAP{text}{margin comment} to add a comment in the margin highlight <text>				%
%	\cmtInAP{text}{comment} to add a comment inline highlight <text>							%
%																								%
%	See http://tug.ctan.org/macros/latex/contrib/todonotes/todonotes.pdf						%
%	for todonotes documentation																	%
%																								%
%	See http://mirrors.ibiblio.org/CTAN/macros/latex/contrib/changes/changes.english.pdf		%
%	for changes documentation																	%
%																								%
%	If you want to define additional authors (10 are already defined} you must					%
%		1. 	define two commands like the one below for each new author							%
%		2. 	add one more \definechangesauthor command for each new author (see below)			%
%		3. 	for each new author add the 7 commands (\delAuth, ecc) to create					%
%			the various commands for track changes and notes  									%
%																								%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%definitions for author 1
\newcommand{\AIid}{AP}
\newcommand{\AIcol}{teal}

%definitions for author 2
\newcommand{\AIIid}{LV}
\newcommand{\AIIcol}{blue}

%definitions for author 3
\newcommand{\AIIIid}{AC}
\newcommand{\AIIIcol}{red}

%definitions for author 4
\newcommand{\AIVid}{AD}
\newcommand{\AIVcol}{brown}

%definitions for author 5
\newcommand{\AVid}{AE}
\newcommand{\AVcol}{darkgray}

%definitions for author 6
\newcommand{\AVIid}{AF}
\newcommand{\AVIcol}{teal}

%definitions for author 7
\newcommand{\AVIIid}{AG}
\newcommand{\AVIIcol}{orange}

%definitions for author 8
\newcommand{\AVIIIid}{AH}
\newcommand{\AVIIIcol}{magenta}

%definitions for author 9
\newcommand{\AIXid}{AI}
\newcommand{\AIXcol}{violet}

%definitions for author 10
\newcommand{\AXid}{AJ}
\newcommand{\AXcol}{olive}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%																								%
% END OF THE PART AUTHORS SHOULD MODIFY															%
% FROM NOW ON, NOTHING SHOULD BE CHANGED, AS EVERYTHING IS AUTOMATIC							%
%																								%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%																								%
% DEFINITION OF THE AUTHORS FOR THE CHANGES PACKAGE - DON'T TOUCH!!!!!!							%
%																								%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\definechangesauthor[color=\AIcol]{\AIid}
\definechangesauthor[color=\AIIcol]{\AIIid}
\definechangesauthor[color=\AIIIcol]{\AIIIid}
\definechangesauthor[color=\AIVcol]{\AIVid}
\definechangesauthor[color=\AVcol]{\AVid}
\definechangesauthor[color=\AVIcol]{\AVIid}
\definechangesauthor[color=\AVIIcol]{\AVIIid}
\definechangesauthor[color=\AVIIIcol]{\AVIIIid}
\definechangesauthor[color=\AIXcol]{\AIXid}
\definechangesauthor[color=\AXcol]{\AXid}

% these macros allow to define the \add, \delXX, \repXX, \cmtXX, \cmtInXX, \todoXX, \todInXX
% commands, where XX are the initials picked by each author

\makeatletter
% for the \del commands
\newcommand{\delAuth}[1]{%
  	\long\@namedef{del#1}##1{\deleted[id=#1]{##1}}%
}
% for the \add commands
\newcommand{\addAuth}[1]{%
  	\long\@namedef{add#1}##1{\added[id=#1]{##1}}%
}
% for the \rep commands
\newcommand{\repAuth}[1]{%
  	\long\@namedef{rep#1}##1##2{\replaced[id=#1]{##1}{##2}}%
}
% for the \todo commands
\newcommand{\todoAuth}[2]{%
  	\long\@namedef{todo#1}##1{%
		\todo[backgroundcolor=white, linecolor=#2, bordercolor=#2,
			size=\small, caption={2do}]{%
				\tiny{%
					\begin{spacing}{0.5}%
						##1%
					\end{spacing}%
				}%
			}%
	}%
}
% for the \todoIn commands
\newcommand{\todoInAuth}[2]{%
  	\long\@namedef{todoIn#1}##1{%
		\todo[backgroundcolor=white, linecolor=#2, bordercolor=#2,
			size=\small, inline, caption={2do}]{%
				\tiny{%
					\begin{spacing}{0.5}%
						##1%
					\end{spacing}%
				}%
			}%
	}%
}
% for the \cmt commands
\newcommand{\cmtAuth}[2]{%
  	\long\@namedef{cmt#1}##1##2{%
		\texthl{##1}%
		\todo[backgroundcolor=white, linecolor=#2, bordercolor=#2,
			size=\small, caption={2do}]{%
				\tiny{%
					\begin{spacing}{0.5}%
						##2%
					\end{spacing}%
				}%
			}%
	}%
}
% for the \cmtIn commands
\newcommand{\cmtInAuth}[2]{%
  	\long\@namedef{cmtIn#1}##1##2{%
		\texthl{##1}%
		\todo[backgroundcolor=white, linecolor=#2, bordercolor=#2,
			size=\small, inline, caption={2do}]{%
				\tiny{%
					\begin{spacing}{0.5}%
						##2%
					\end{spacing}%
				}%
			}%
	}%
}
\makeatother



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%																								%
% CREATION OF ALL COMMANDS FOR ALL AUTHORS - DON'T TOUCH!!!!!!									%
%																								%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Author 1
\delAuth{\AIid}
\addAuth{\AIid}
\repAuth{\AIid}
\todoAuth{\AIid}{\AIcol}
\todoInAuth{\AIid}{\AIcol}
\cmtAuth{\AIid}{\AIcol}
\cmtInAuth{\AIid}{\AIcol}

% Author 2
\delAuth{\AIIid}
\addAuth{\AIIid}
\repAuth{\AIIid}
\todoAuth{\AIIid}{\AIIcol}
\todoInAuth{\AIIid}{\AIIcol}
\cmtAuth{\AIIid}{\AIIcol}
\cmtInAuth{\AIIid}{\AIIcol}

% Author 3
\delAuth{\AIIIid}
\addAuth{\AIIIid}
\repAuth{\AIIIid}
\todoAuth{\AIIIid}{\AIIIcol}
\todoInAuth{\AIIIid}{\AIIIcol}
\cmtAuth{\AIIIid}{\AIIIcol}
\cmtInAuth{\AIIIid}{\AIIIcol}

% Author 4
\delAuth{\AIVid}
\addAuth{\AIVid}
\repAuth{\AIVid}
\todoAuth{\AIVid}{\AIVcol}
\todoInAuth{\AIVid}{\AIVcol}
\cmtAuth{\AIVid}{\AIVcol}
\cmtInAuth{\AIVid}{\AIVcol}

% Author 5
\delAuth{\AVid}
\addAuth{\AVid}
\repAuth{\AVid}
\todoAuth{\AVid}{\AVcol}
\todoInAuth{\AVid}{\AVcol}
\cmtAuth{\AVid}{\AVcol}
\cmtInAuth{\AVid}{\AVcol}

% Author 6
\delAuth{\AVIid}
\addAuth{\AVIid}
\repAuth{\AVIid}
\todoAuth{\AVIid}{\AVIcol}
\todoInAuth{\AVIid}{\AVIcol}
\cmtAuth{\AIid}{\AIcol}
\cmtInAuth{\AIid}{\AIcol}

% Author 7
\delAuth{\AVIIid}
\addAuth{\AVIIid}
\repAuth{\AIid}
\todoAuth{\AVIIid}{\AVIIcol}
\todoInAuth{\AVIIid}{\AVIIcol}
\cmtAuth{\AVIIid}{\AVIIcol}
\cmtInAuth{\AVIIid}{\AVIIcol}

% Author 8
\delAuth{\AVIIid}
\addAuth{\AVIIIid}
\repAuth{\AVIIIid}
\todoAuth{\AVIIIid}{\AIIIcol}
\todoInAuth{\AVIIIid}{\AVIIIcol}
\cmtAuth{\AVIIIid}{\AVIIIcol}
\cmtInAuth{\AVIIIid}{\AVIIIcol}

% Author 9
\delAuth{\AIXid}
\addAuth{\AIXid}
\repAuth{\AIXid}
\todoAuth{\AIXid}{\AIXcol}
\todoInAuth{\AIXid}{\AIXcol}
\cmtAuth{\AIXid}{\AIXcol}
\cmtInAuth{\AIXid}{\AIXcol}

% Author 10
\delAuth{\AXid}
\addAuth{\AXid}
\repAuth{\AXid}
\todoAuth{\AXid}{\AXcol}
\todoInAuth{\AXid}{\AXcol}
\cmtAuth{\AXid}{\AXcol}
\cmtInAuth{\AXid}{\AXcol}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%																								%
% OK, NOW YOU CAN DO WHATEVER YOU WANT (UNDER YOUR RESPONSIBILITY...)							%
%																								%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

